S2MDF: A Plug-And-Play Layer for Intersection-Free Multi-Object Signed Distance Fields

Compositional implicit surface representations model scenes as collections of objects, each encoded by a Signed Distance Field (SDF). A fundamental limitation of this approach is that multiple SDFs can produce geometries that interpenetrate, violating physical plausibility. Existing mitigation strategies rely on soft penalty terms that reduce but do not eliminate intersections, and require careful loss weighting. To truly prevent interpenetration, we propose a hard constraint on vector-valued SDFs and introduce S2MDF, a lightweight plug-and-play module that enforces the constraint on any object-compositional SDF representation without architectural modifications. It introduces negligible computational overhead and is compatible with linearly-interpolated standard meshing algorithms such as Marching Cubes. It can be applied during training or as a post-processing step. Experiments on multiple state-of-the-art compositional methods show that S2MDF reduces intersections to numerical precision while preserving reconstruction quality, outperforming existing mitigation strategies.

==> tabs/medtet/heart/mean.tex <==
\begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|cccc}
    \toprule
     & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ \\
    \midrule
    Default & $23.863 \ (\times 10^{-4})$ & $0.943$ & $0.975$ & $3.445 \ (\times 10^{-4})$ \\
    QP (Training) & $24.796 \ (\times 10^{-4})$ & $0.944$ & $0.975$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PP) & $29.420 \ (\times 10^{-4})$ & $0.943$ & $0.974$ & $0.000 \ (\times 10^{-4})$ \\
    Shiftall (Training) & $23.094 \ (\times 10^{-4})$ & $0.944$ & $0.976$ & $0.000 \ (\times 10^{-4})$ \\
    Shiftall (PP) & $31.099 \ (\times 10^{-4})$ & $0.943$ & $0.973$ & $0.000 \ (\times 10^{-4})$ \\
    \bottomrule
  \end{tabular}%
  }
\caption{MedTet trained on 15 complete hearts, tested on 5. Mean metrics across shapes and lobes. Standard deviation over 3 different seeds.}
\label{tab:medtet_lung_mean}%
\end{table}


==> tabs/medtet/heart/std.tex <==
\begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|cccc}
    \toprule
     & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ \\
    \midrule
    Default & $1.330 \ (\times 10^{-4})$ & $0.002$ & $0.001$ & $1.390 \ (\times 10^{-4})$ \\
    QP (Training) & $0.670 \ (\times 10^{-4})$ & $0.001$ & $0.003$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PP) & $4.430 \ (\times 10^{-4})$ & $0.001$ & $0.001$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PC+Training) & $0.000 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PC+PP) & $1.411 \ (\times 10^{-4})$ & $0.002$ & $0.002$ & $0.000 \ (\times 10^{-4})$ \\
    Shiftall (Training) & $0.331 \ (\times 10^{-4})$ & $0.001$ & $0.002$ & $0.000 \ (\times 10^{-4})$ \\
    Shiftall (PP) & $7.072 \ (\times 10^{-4})$ & $0.002$ & $0.002$ & $0.000 \ (\times 10^{-4})$ \\
    \bottomrule
  \end{tabular}%
  }
\end{table}



==> tabs/medtet/left_lung/all.tex <==
% Small model (final, 5 seeds)
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|cccccc}
%     \toprule
%      & MCD & MNC & F1 (0.01) & IV & PCD (0.01) & IoU \\
%     \midrule
%     Vanilla & $6.2696 \pm 0.2011 \ (\times 10^{-4})$ & $0.9581 \pm 0.0004$ & $0.9949 \pm 0.0003$ & $0.2282 \pm 0.1060 \ (\times 10^{-4})$ & $14.7463 \pm 0.2433 \ (\times 10^{-4})$ & $0.4172 \pm 0.0004$ \\
%     QP (Training) & $6.0958 \pm 0.3433 \ (\times 10^{-4})$ & $0.9581 \pm 0.0005$ & $0.9951 \pm 0.0004$ & $0.0000 \pm 0.0000 \ (\times 10^{-4})$ & $14.5678 \pm 0.7255 \ (\times 10^{-4})$ & $0.4175 \pm 0.0005$ \\
%     QP (PP) & $6.4775 \pm 0.3201 \ (\times 10^{-4})$ & $0.9579 \pm 0.0008$ & $0.9947 \pm 0.0004$ & $0.0000 \pm 0.0000 \ (\times 10^{-4})$ & $15.2621 \pm 0.6554 \ (\times 10^{-4})$ & $0.4173 \pm 0.0007$ \\
%     Shiftall (Training) & $6.4694 \pm 0.4791 \ (\times 10^{-4})$ & $0.9582 \pm 0.0007$ & $0.9948 \pm 0.0005$ & $0.0000 \pm 0.0000 \ (\times 10^{-4})$ & $14.9662 \pm 0.7499 \ (\times 10^{-4})$ & $0.4173 \pm 0.0003$ \\
%     Shiftall (PP) & $6.2994 \pm 0.5489 \ (\times 10^{-4})$ & $0.9581 \pm 0.0003$ & $0.9949 \pm 0.0004$ & $0.0000 \pm 0.0000 \ (\times 10^{-4})$ & $14.7259 \pm 0.8120 \ (\times 10^{-4})$ & $0.4173 \pm 0.0003$ \\
%     \bottomrule
%   \end{tabular}%
%   }


% Full model (best, 3 seeds)
\begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|cccccc}
    \toprule
     & MCD & MNC & F1 (0.01) & IV & PCD (0.01) & IoU \\
    \midrule
    Default & $5.1584 \pm 0.1457 \ (\times 10^{-4})$ & $0.9702 \pm 0.0006$ & $0.9956 \pm 0.0002$ & $1.7290 \pm 0.6804 \ (\times 10^{-4})$ & $12.5784 \pm 0.8133 \ (\times 10^{-4})$ & $0.0001 \pm 0.0000$ \\
    QP (Training) & $5.1077 \pm 0.0555 \ (\times 10^{-4})$ & $0.9698 \pm 0.0009$ & $0.9956 \pm 0.0001$ & $0.0024 \pm 0.0029 \ (\times 10^{-4})$ & $12.6538 \pm 0.2221 \ (\times 10^{-4})$ & $0.0001 \pm 0.0000$ \\
    QP (PP) & $5.2364 \pm 0.1248 \ (\times 10^{-4})$ & $0.9699 \pm 0.0012$ & $0.9956 \pm 0.0001$ & $0.0016 \pm 0.0022 \ (\times 10^{-4})$ & $12.8308 \pm 1.3545 \ (\times 10^{-4})$ & $0.0001 \pm 0.0001$ \\
    QP (PC+Training) & $5.1515 \pm 0.0735 \ (\times 10^{-4})$ & $0.9697 \pm 0.0003$ & $0.9957 \pm 0.0000$ & $0.0012 \pm 0.0007 \ (\times 10^{-4})$ & $13.1659 \pm 0.4811 \ (\times 10^{-4})$ & $0.0001 \pm 0.0000$ \\
    QP (PC+PP) & $4.9526 \pm 0.1054 \ (\times 10^{-4})$ & $0.9700 \pm 0.0006$ & $0.9957 \pm 0.0002$ & $0.0058 \pm 0.0058 \ (\times 10^{-4})$ & $12.2428 \pm 1.3030 \ (\times 10^{-4})$ & $0.0001 \pm 0.0000$ \\
    Shiftall (Training) & $5.3048 \pm 0.1475 \ (\times 10^{-4})$ & $0.9703 \pm 0.0008$ & $0.9957 \pm 0.0001$ & $0.0005 \pm 0.0005 \ (\times 10^{-4})$ & $13.4649 \pm 0.8339 \ (\times 10^{-4})$ & $0.0001 \pm 0.0000$ \\
    Shiftall (PP) & $5.2032 \pm 0.2045 \ (\times 10^{-4})$ & $0.9699 \pm 0.0013$ & $0.9956 \pm 0.0003$ & $0.0124 \pm 0.0090 \ (\times 10^{-4})$ & $13.1203 \pm 0.8573 \ (\times 10^{-4})$ & $0.0001 \pm 0.0000$ \\
    \bottomrule
  \end{tabular}%
  }

% Full model (final, 3 seeds)
% \begin{table}[t]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|cccccc}
%     \toprule
%      & MCD & MNC & F1 (0.01) & IV & PCD (0.01) & IoU \\
%     \midrule
%     Default & $(5.6360 \pm 0.5411) \times 10^{-4}$ & $0.9704 \pm 0.0004$ & $0.9952 \pm 0.0002$ & $(1.1232 \pm 1.0949) \times 10^{-4}$ & $(13.3624 \pm 1.4882) \times 10^{-4}$ & $0.0001 \pm 0.0000$ \\
%     QP (Training) & $(5.9358 \pm 0.2685) \times 10^{-4}$ & $0.9705 \pm 0.0004$ & $0.9952 \pm 0.0002$ & $(0.0024 \pm 0.0025) \times 10^{-4}$ & $(14.7400 \pm 0.3827) \times 10^{-4}$ & $0.0001 \pm 0.0000$ \\
%     QP (PP) & $(5.8450 \pm 0.2455) \times 10^{-4}$ & $0.9701 \pm 0.0003$ & $0.9952 \pm 0.0001$ & $(0.0082 \pm 0.0123) \times 10^{-4}$ & $(14.0873 \pm 0.2557) \times 10^{-4}$ & $0.0001 \pm 0.0000$ \\
%     QP (PC+Training) & $(6.1462 \pm 1.1837) \times 10^{-4}$ & $0.9673 \pm 0.0061$ & $0.9952 \pm 0.0004$ & $(0.0008 \pm 0.0009) \times 10^{-4}$ & $(14.5999 \pm 1.1295) \times 10^{-4}$ & $0.0001 \pm 0.0000$ \\
%     QP (PC+PP) & $(6.8568 \pm 2.3817) \times 10^{-4}$ & $0.9694 \pm 0.0015$ & $0.9949 \pm 0.0008$ & $(0.0021 \pm 0.0009) \times 10^{-4}$ & $(14.4686 \pm 1.6491) \times 10^{-4}$ & $0.0001 \pm 0.0000$ \\
%     Shiftall (Training) & $(6.2749 \pm 0.5360) \times 10^{-4}$ & $0.9696 \pm 0.0003$ & $0.9946 \pm 0.0007$ & $(0.0016 \pm 0.0004) \times 10^{-4}$ & $(14.8978 \pm 1.5712) \times 10^{-4}$ & $0.0001 \pm 0.0000$ \\
%     Shiftall (PP) & $(6.1957 \pm 0.4284) \times 10^{-4}$ & $0.9703 \pm 0.0003$ & $0.9949 \pm 0.0001$ & $(0.0064 \pm 0.0070) \times 10^{-4}$ & $(14.7952 \pm 0.3901) \times 10^{-4}$ & $0.0001 \pm 0.0000$ \\
%     \bottomrule
%   \end{tabular}%
%   }
\caption{MedTet trained on 200 left lungs with two lobes, tested on 118. Mean metrics across shapes and lobes. Standard deviation over 3 different seeds.}
\label{tab:supp_medtet_leftlung}%
\end{table}


==> tabs/medtet/left_lung/mean.tex <==
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|ccccc}
%     \toprule
%      & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
%     \midrule
%     Default & $5.636 \ (\times 10^{-4})$ & $0.970$ & $0.995$ & $13.362 \ (\times 10^{-4})$ & $1.123 \ (\times 10^{-4})$ \\
%     QP (Training) & $5.936 \ (\times 10^{-4})$ & $0.971$ & $0.995$ & $14.740 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
%     QP (PP) & $5.845 \ (\times 10^{-4})$ & $0.970$ & $0.995$ & $14.087 \ (\times 10^{-4})$ & $0.008 \ (\times 10^{-4})$ \\
%     QP (PC+Training) & $6.146 \ (\times 10^{-4})$ & $0.967$ & $0.995$ & $14.600 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
%     QP (PC+PP) & $6.857 \ (\times 10^{-4})$ & $0.969$ & $0.995$ & $14.469 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
%     Shiftall (Training) & $6.275 \ (\times 10^{-4})$ & $0.970$ & $0.995$ & $14.898 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
%     Shiftall (PP) & $6.196 \ (\times 10^{-4})$ & $0.970$ & $0.995$ & $14.795 \ (\times 10^{-4})$ & $0.006 \ (\times 10^{-4})$ \\
%     \bottomrule
%   \end{tabular}%
%   }

% Best
  \begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|ccccc}
    \toprule
     & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
    \midrule
    Default & $5.158 \ (\times 10^{-4})$ & $0.970$ & $0.996$ & $12.578 \ (\times 10^{-4})$ & $1.729 \ (\times 10^{-4})$ \\
    QP (Training) & $5.108 \ (\times 10^{-4})$ & $0.970$ & $0.996$ & $12.654 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
    QP (PP) & $5.236 \ (\times 10^{-4})$ & $0.970$ & $0.996$ & $12.831 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
    % QP (PC+Training) & $5.152 \ (\times 10^{-4})$ & $0.970$ & $0.996$ & $13.166 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
    % QP (PC+PP) & $4.953 \ (\times 10^{-4})$ & $0.970$ & $0.996$ & $12.243 \ (\times 10^{-4})$ & $0.006 \ (\times 10^{-4})$ \\
    Shiftall (Training) & $5.305 \ (\times 10^{-4})$ & $0.970$ & $0.996$ & $13.465 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    Shiftall (PP) & $5.203 \ (\times 10^{-4})$ & $0.970$ & $0.996$ & $13.120 \ (\times 10^{-4})$ & $0.012 \ (\times 10^{-4})$ \\
    \bottomrule
  \end{tabular}%
  }

% Small
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|ccccc}
%     \toprule
%      & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
%     \midrule
%     Vanilla & $6.270 \ (\times 10^{-4})$ & $0.958$ & $0.995$ & $14.746 \ (\times 10^{-4})$ & $0.228 \ (\times 10^{-4})$ \\
%     QP (Training) & $6.096 \ (\times 10^{-4})$ & $0.958$ & $0.995$ & $14.568 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
%     QP (PP) & $6.478 \ (\times 10^{-4})$ & $0.958$ & $0.995$ & $15.262 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
%     QP (PC+Training) & $6.166 \ (\times 10^{-4})$ & $0.958$ & $0.995$ & $14.669 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
%     QP (PC+PP) & $6.406 \ (\times 10^{-4})$ & $0.958$ & $0.995$ & $15.202 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
%     Shiftall (Training) & $6.469 \ (\times 10^{-4})$ & $0.958$ & $0.995$ & $14.966 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
%     Shiftall (PP) & $6.299 \ (\times 10^{-4})$ & $0.958$ & $0.995$ & $14.726 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
%     \bottomrule
%   \end{tabular}%
%   }


\caption{MedTet trained on 200 left lungs with two lobes, tested on 118. Mean metrics across shapes and lobes. Standard deviation over 3 different seeds.}
\label{tab:medtet_leftlung_mean}%
\end{table}


==> tabs/medtet/left_lung/std.tex <==
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|ccccc}
%     \toprule
%      & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
%     \midrule
%     Default & $0.541 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $1.488 \ (\times 10^{-4})$ & $1.095 \ (\times 10^{-4})$ \\
%     QP (Training) & $0.269 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.383 \ (\times 10^{-4})$ & $0.003 \ (\times 10^{-4})$ \\
%     QP (PP) & $0.246 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.256 \ (\times 10^{-4})$ & $0.012 \ (\times 10^{-4})$ \\
%     QP (PC+Training) & $1.184 \ (\times 10^{-4})$ & $0.006$ & $0.000$ & $1.130 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
%     QP (PC+PP) & $2.382 \ (\times 10^{-4})$ & $0.002$ & $0.001$ & $1.649 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
%     Shiftall (Training) & $0.536 \ (\times 10^{-4})$ & $0.000$ & $0.001$ & $1.571 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
%     Shiftall (PP) & $0.428 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.390 \ (\times 10^{-4})$ & $0.007 \ (\times 10^{-4})$ \\
%     \bottomrule
%   \end{tabular}%
%   }

  % Best
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|ccccc}
%     \toprule
%      & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
%     \midrule
%     Default & $0.146 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.813 \ (\times 10^{-4})$ & $0.680 \ (\times 10^{-4})$ \\
%     QP (Training) & $0.056 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.222 \ (\times 10^{-4})$ & $0.003 \ (\times 10^{-4})$ \\
%     QP (PP) & $0.125 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $1.355 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
%     QP (PC+Training) & $0.074 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.481 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
%     QP (PC+PP) & $0.105 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $1.303 \ (\times 10^{-4})$ & $0.006 \ (\times 10^{-4})$ \\
%     Shiftall (Training) & $0.147 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.834 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
%     Shiftall (PP) & $0.205 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.857 \ (\times 10^{-4})$ & $0.009 \ (\times 10^{-4})$ \\
%     \bottomrule
%   \end{tabular}%
%   }


% Small
\begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|ccccc}
    \toprule
     & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
    \midrule
    Vanilla & $0.201 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.243 \ (\times 10^{-4})$ & $0.106 \ (\times 10^{-4})$ \\
    QP (Training) & $0.343 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.725 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PP) & $0.320 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.655 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PC+Training) & $0.401 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.890 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PC+PP) & $0.273 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.656 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    Shiftall (Training) & $0.479 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.750 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    Shiftall (PP) & $0.549 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.812 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    \bottomrule
  \end{tabular}%

\caption{MedTet trained on 200 left lungs with two lobes, tested on 118. Mean metrics across shapes and lobes. Standard deviation over 3 different seeds.}
\label{tab:medtet_leftlung_std}%
\end{table}



==> tabs/medtet/lung/all.tex <==


% Full model (best, 3 seeds)
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|cccccc}
%     \toprule
%      & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ & PCD (0.01) $\downarrow$ & IoU $\uparrow$ \\
%     \midrule
%     Default & $5.3812 \pm 0.0603 \ (\times 10^{-4})$ & $0.9665 \pm 0.0012$ & $0.9960 \pm 0.0001$ & $2.7931 \pm 0.8285 \ (\times 10^{-4})$ & $10.6507 \pm 0.2552 \ (\times 10^{-4})$ & $0.0006 \pm 0.0001$ \\
%     QP (Training) & $5.3555 \pm 0.3065 \ (\times 10^{-4})$ & $0.9679 \pm 0.0002$ & $0.9959 \pm 0.0001$ & $0.0019 \pm 0.0004 \ (\times 10^{-4})$ & $11.0291 \pm 0.3418 \ (\times 10^{-4})$ & $0.0006 \pm 0.0000$ \\
%     QP (PP) & $5.8030 \pm 0.3202 \ (\times 10^{-4})$ & $0.9677 \pm 0.0000$ & $0.9958 \pm 0.0004$ & $0.0119 \pm 0.0041 \ (\times 10^{-4})$ & $11.4532 \pm 0.3844 \ (\times 10^{-4})$ & $0.0005 \pm 0.0000$ \\
%     QP (PC+Training) & $5.3976 \pm 0.0000 \ (\times 10^{-4})$ & $0.9679 \pm 0.0000$ & $0.9963 \pm 0.0000$ & $0.0022 \pm 0.0000 \ (\times 10^{-4})$ & $10.6316 \pm 0.0000 \ (\times 10^{-4})$ & $0.0006 \pm 0.0000$ \\
%     Shiftall (Training) & $5.3921 \pm 0.0559 \ (\times 10^{-4})$ & $0.9679 \pm 0.0006$ & $0.9962 \pm 0.0001$ & $0.0014 \pm 0.0009 \ (\times 10^{-4})$ & $10.7889 \pm 0.1911 \ (\times 10^{-4})$ & $0.0006 \pm 0.0001$ \\
%     Shiftall (PP) & $5.5086 \pm 0.3484 \ (\times 10^{-4})$ & $0.9671 \pm 0.0003$ & $0.9959 \pm 0.0005$ & $0.0103 \pm 0.0023 \ (\times 10^{-4})$ & $10.9174 \pm 0.4527 \ (\times 10^{-4})$ & $0.0006 \pm 0.0001$ \\
%     \bottomrule
%   \end{tabular}%
%   }


% Full model (final, 3 seeds)
\begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|cccccc}
    \toprule
     & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ & PCD (0.01) $\downarrow$ & IoU $\uparrow$ \\
    \midrule
    Default & $5.4621 \pm 0.1184 \ (\times 10^{-4})$ & $0.9673 \pm 0.0006$ & $0.9960 \pm 0.0001$ & $2.7550 \pm 0.7666 \ (\times 10^{-4})$ & $10.8927 \pm 0.1698 \ (\times 10^{-4})$ & $0.0006 \pm 0.0001$ \\
    QP (Training) & $5.3569 \pm 0.3090 \ (\times 10^{-4})$ & $0.9679 \pm 0.0002$ & $0.9959 \pm 0.0001$ & $0.0019 \pm 0.0004 \ (\times 10^{-4})$ & $11.0277 \pm 0.3426 \ (\times 10^{-4})$ & $0.0006 \pm 0.0000$ \\
    QP (PP) & $5.7998 \pm 0.3142 \ (\times 10^{-4})$ & $0.9677 \pm 0.0000$ & $0.9958 \pm 0.0003$ & $0.0119 \pm 0.0041 \ (\times 10^{-4})$ & $11.4482 \pm 0.3964 \ (\times 10^{-4})$ & $0.0005 \pm 0.0000$ \\
    QP (PC+Training) & $5.4705 \pm 0.0847 \ (\times 10^{-4})$ & $0.9683 \pm 0.0004$ & $0.9960 \pm 0.0003$ & $0.0021 \pm 0.0014 \ (\times 10^{-4})$ & $11.1393 \pm 0.6535 \ (\times 10^{-4})$ & $0.0006 \pm 0.0002$ \\
    QP (PC+PP) & $5.7076 \pm 0.0549 \ (\times 10^{-4})$ & $0.9674 \pm 0.0008$ & $0.9958 \pm 0.0002$ & $0.0065 \pm 0.0018 \ (\times 10^{-4})$ & $11.2857 \pm 0.2569 \ (\times 10^{-4})$ & $0.0005 \pm 0.0001$ \\
    Shiftall (Training) & $5.3935 \pm 0.0557 \ (\times 10^{-4})$ & $0.9679 \pm 0.0006$ & $0.9962 \pm 0.0001$ & $0.0014 \pm 0.0009 \ (\times 10^{-4})$ & $10.7890 \pm 0.1862 \ (\times 10^{-4})$ & $0.0006 \pm 0.0001$ \\
    Shiftall (PP) & $5.5997 \pm 0.2889 \ (\times 10^{-4})$ & $0.9671 \pm 0.0002$ & $0.9958 \pm 0.0004$ & $0.0113 \pm 0.0024 \ (\times 10^{-4})$ & $11.0324 \pm 0.3798 \ (\times 10^{-4})$ & $0.0005 \pm 0.0001$ \\
    \bottomrule
  \end{tabular}%
  }

\caption{MedTet trained on 200 complete lungs, tested on 118. Mean metrics across shapes and lobes. Standard deviation over 3 different seeds.}
\label{tab:supp_medtet_lung}%
\end{table}


==> tabs/medtet/lung/mean.tex <==
% Final
\begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|ccccc}
    \toprule
     & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
    \midrule
    Default & $5.462 \ (\times 10^{-4})$ & $0.967$ & $0.996$ & $10.893 \ (\times 10^{-4})$ & $2.755 \ (\times 10^{-4})$ \\
    QP (Training) & $5.357 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $11.028 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
    QP (PP) & $5.800 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $11.448 \ (\times 10^{-4})$ & $0.012 \ (\times 10^{-4})$ \\
    % QP (PC+Training) & $5.471 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $11.139 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
    % QP (PC+PP) & $5.708 \ (\times 10^{-4})$ & $0.967$ & $0.996$ & $11.286 \ (\times 10^{-4})$ & $0.006 \ (\times 10^{-4})$ \\
    Shiftall (Training) & $5.394 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $10.789 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
    Shiftall (PP) & $5.600 \ (\times 10^{-4})$ & $0.967$ & $0.996$ & $11.032 \ (\times 10^{-4})$ & $0.011 \ (\times 10^{-4})$ \\
    \bottomrule
  \end{tabular}%
  }


% % Best
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|cccccc}
%     \toprule
%      & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ & PCD (0.01) $\downarrow$ & IoU $\uparrow$ \\
%     \midrule
%     Default & $5.381 \ (\times 10^{-4})$ & $0.967$ & $0.996$ & $2.793 \ (\times 10^{-4})$ & $10.651 \ (\times 10^{-4})$ & $0.001$ \\
%     QP (Training) & $5.355 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $0.002 \ (\times 10^{-4})$ & $11.029 \ (\times 10^{-4})$ & $0.001$ \\
%     QP (PP) & $5.803 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $0.012 \ (\times 10^{-4})$ & $11.453 \ (\times 10^{-4})$ & $0.001$ \\
%     QP (PC+Training) & $5.398 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $0.002 \ (\times 10^{-4})$ & $10.632 \ (\times 10^{-4})$ & $0.001$ \\
%     Shiftall (Training) & $5.392 \ (\times 10^{-4})$ & $0.968$ & $0.996$ & $0.001 \ (\times 10^{-4})$ & $10.789 \ (\times 10^{-4})$ & $0.001$ \\
%     Shiftall (PP) & $5.509 \ (\times 10^{-4})$ & $0.967$ & $0.996$ & $0.010 \ (\times 10^{-4})$ & $10.917 \ (\times 10^{-4})$ & $0.001$ \\
%     \bottomrule
%   \end{tabular}%
%   }
\caption{MedTet trained on 200 complete lungs, tested on 118. Mean metrics across shapes and lobes. Standard deviation over 3 different seeds.}
\label{tab:medtet_lung_mean}%
\end{table}



==> tabs/medtet/lung/std.tex <==
% Last
\begin{table}[ht]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|ccccc}
    \toprule
     & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & PCD (0.01) $\downarrow$ & IV $\downarrow$ \\
    \midrule
    Default & $0.118 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.170 \ (\times 10^{-4})$ & $0.767 \ (\times 10^{-4})$ \\
    QP (Training) & $0.309 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.343 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ \\
    QP (PP) & $0.314 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.396 \ (\times 10^{-4})$ & $0.004 \ (\times 10^{-4})$ \\
    QP (PC+Training) & $0.085 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.654 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
    QP (PC+PP) & $0.055 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.257 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
    Shiftall (Training) & $0.056 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.186 \ (\times 10^{-4})$ & $0.001 \ (\times 10^{-4})$ \\
    Shiftall (PP) & $0.289 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.380 \ (\times 10^{-4})$ & $0.002 \ (\times 10^{-4})$ \\
    \bottomrule
  \end{tabular}%
  }

% Best
% \begin{table}[ht]
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \begin{tabular}{l|cccccc}
%     \toprule
%      & MCD $\downarrow$ & MNC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ & PCD (0.01) $\downarrow$ & IoU $\uparrow$ \\
%     \midrule
%     Default & $0.060 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.829 \ (\times 10^{-4})$ & $0.255 \ (\times 10^{-4})$ & $0.000$ \\
%     QP (Training) & $0.306 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.000 \ (\times 10^{-4})$ & $0.342 \ (\times 10^{-4})$ & $0.000$ \\
%     QP (PP) & $0.320 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.004 \ (\times 10^{-4})$ & $0.384 \ (\times 10^{-4})$ & $0.000$ \\
%     QP (PC+Training) & $0.000 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.000 \ (\times 10^{-4})$ & $0.000 \ (\times 10^{-4})$ & $0.000$ \\
%     Shiftall (Training) & $0.056 \ (\times 10^{-4})$ & $0.001$ & $0.000$ & $0.001 \ (\times 10^{-4})$ & $0.191 \ (\times 10^{-4})$ & $0.000$ \\
%     Shiftall (PP) & $0.348 \ (\times 10^{-4})$ & $0.000$ & $0.000$ & $0.002 \ (\times 10^{-4})$ & $0.453 \ (\times 10^{-4})$ & $0.000$ \\
%     \bottomrule
%   \end{tabular}%
%   }
\end{table}



==> tabs/partsdf_chair100.tex <==
% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|cccc}
%      & MCD $\downarrow$ & NC $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
%     \hline
%     Vanilla PartSDF & 3.567 $\pm$ 13.130 & 95.107 $\pm$ 4.402 & 85.716 $\pm$ 10.951 & (1.788 $\pm$ 5.729) $\times 10^{-3}$ \\
%     \hline
%     % Min - PP (MC) & 2.249 $\pm$ 12.658 & 94.743 $\pm$ 4.473 & 89.209 $\pm$ 9.618 & (1.454 $\pm$ 3.146) $\times 10^{-7}$ \\
%     S2MDF (QP) - PP & 2.305 $\pm$ 12.704 & 94.791 $\pm$ 4.483 & 89.186 $\pm$ 9.604 & (6.139 $\pm$ 34.630) $\times 10^{-9}$ \\
%     S2MDF (Shift-All) - PP & 2.206 $\pm$ 12.680 & 94.834 $\pm$ 4.472 & 89.207 $\pm$ 9.606 & (6.663 $\pm$ 30.730) $\times 10^{-9}$ \\
%     % \hline
%     % Min - Optim (MC) & 2.244 $\pm$ 10.445 & 94.708 $\pm$ 4.579 & 89.071 $\pm$ 9.570 & (1.681 $\pm$ 3.408) $\times 10^{-7}$ \\
%     % Shift - Optim (MC) & 2.838 $\pm$ 21.485 & 94.898 $\pm$ 4.474 & 89.686 $\pm$ 9.737 & (3.550 $\pm$ 32.310) $\times 10^{-9}$ \\
%     % QP - Optim (MC) & 2.801 $\pm$ 20.365 & 94.871 $\pm$ 4.388 & 89.628 $\pm$ 9.801 & (4.145 $\pm$ 27.200) $\times 10^{-9}$ \\
%     \hline
%     % Min - Train (MC) & 2.347 $\pm$ 12.954 & 94.727 $\pm$ 4.474 & 89.043 $\pm$ 9.406 & (1.398 $\pm$ 3.071) $\times 10^{-7}$ \\
%     S2MDF (QP) - Train & 2.700 $\pm$ 18.035 & 94.991 $\pm$ 4.085 & 89.416 $\pm$ 9.361 & (8.117 $\pm$ 40.900) $\times 10^{-9}$ \\
%     S2MDF (Shift-All) - Train & 2.173 $\pm$ 11.984 & 94.800 $\pm$ 4.437 & 89.196 $\pm$ 9.407 & (7.320 $\pm$ 26.150) $\times 10^{-9}$ \\
%   \end{tabular}%
% }
% \caption{PartSDF trained on 100 chairs, tested on different 100 chairs. Mean metrics across shapes and parts.}
% \label{tab:partsdf_chair100}%
% \end{table}


\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{c|cccc}
     & MCD $\downarrow$ & NC $\uparrow$ & F1 (0.001) $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
    \hline
    Vanilla PartSDF & 3.567 $\pm$ 13.130 & 95.107 $\pm$ 4.402 & 85.716 $\pm$ 10.951 & (1.788 $\pm$ 5.729) $\times 10^{-3}$ \\
    \hline
    S2MDF (QP) - PP & 2.305 $\pm$ 12.704 & 94.791 $\pm$ 4.483 & 89.186 $\pm$ 9.604 & (6.139 $\pm$ 34.630) $\times 10^{-9}$ \\
    S2MDF (Shift-All) - PP & 2.206 $\pm$ 12.680 & 94.834 $\pm$ 4.472 & 89.207 $\pm$ 9.606 & (6.663 $\pm$ 30.730) $\times 10^{-9}$ \\
    \hline
    S2MDF (QP) - Train & 2.700 $\pm$ 18.035 & 94.991 $\pm$ 4.085 & 89.416 $\pm$ 9.361 & (8.117 $\pm$ 40.900) $\times 10^{-9}$ \\
    S2MDF (Shift-All) - Train & 2.173 $\pm$ 11.984 & 94.800 $\pm$ 4.437 & 89.196 $\pm$ 9.407 & (7.320 $\pm$ 26.150) $\times 10^{-9}$ \\
  \end{tabular}%
}
\caption{PartSDF trained on 100 chairs, tested on different 100 chairs. Mean metrics across shapes and parts.}
\label{tab:partsdf_chair100}%
\end{table}

==> tabs/partsdf_mixer100.tex <==
% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|cccc}
%     & MCD $\downarrow$ & NC $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
%     \hline
%     Vanilla PartSDF & 1.298 $\pm$ 6.284 & 88.102 $\pm$ 12.363 & 76.667 $\pm$ 23.994 & (4.005 $\pm$ 7.699) $\times 10^{-5}$ \\
%     \hline
%     % Min - PP (MC) & 1.296 $\pm$ 6.284 & 88.182 $\pm$ 12.416 & 76.734 $\pm$ 24.043 & (1.470 $\pm$ 5.412) $\times 10^{-7}$ \\
%     S2MDF (QP) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.447 & 75.812 $\pm$ 24.337 & (1.333 $\pm$ 4.423) $\times 10^{-7}$ \\
%     S2MDF (Shift-All) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.448 & 75.812 $\pm$ 24.337 & (1.337 $\pm$ 4.428) $\times 10^{-7}$ \\
%     % \hline
%     % Min - Optim (MC) & 1.298 $\pm$ 6.290 & 88.178 $\pm$ 12.441 & 76.729 $\pm$ 24.055 & (1.211 $\pm$ 4.632) $\times 10^{-7}$ \\
%     % Shift - Optim (MC) & 1.296 $\pm$ 6.208 & 88.137 $\pm$ 12.392 & 76.483 $\pm$ 24.039 & (3.974 $\pm$ 28.770) $\times 10^{-9}$ \\
%     % QP - Optim (MC) & 1.303 $\pm$ 6.240 & 88.129 $\pm$ 12.405 & 76.482 $\pm$ 24.037 & (4.101 $\pm$ 28.890) $\times 10^{-9}$ \\
%     \hline
%     % Min - Train (MC) & 1.497 $\pm$ 7.075 & 88.133 $\pm$ 12.645 & 76.801 $\pm$ 24.015 & (3.740 $\pm$ 19.160) $\times 10^{-9}$ \\
%     S2MDF (QP) - Train & 1.289 $\pm$ 6.767 & 88.032 $\pm$ 12.619 & 76.419 $\pm$ 24.389 & (6.174 $\pm$ 25.820) $\times 10^{-9}$ \\
%     S2MDF (Shift-All) - Train & 1.161 $\pm$ 5.533 & 88.137 $\pm$ 12.256 & 76.435 $\pm$ 24.276 & (2.418 $\pm$ 11.320) $\times 10^{-8}$ \\
%   \end{tabular}%
% }
% \caption{PartSDF trained on 100 mixers, tested on different 100 mixers. Mean metrics across shapes and parts.}
% \label{tab:partsdf_mixer100}
% \end{table}


% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|ccccc}
%     & MCD $(\times 10^{-4})$ $\downarrow$ & NC $\uparrow$ & F1 (0.001) $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
%     \hline
%     Vanilla PartSDF & 1.298 $\pm$ 6.284 & 88.102 $\pm$ 12.363 & 98.481 $\pm$ 7.898 & 76.667 $\pm$ 23.994 & (4.005 $\pm$ 7.699) $\times 10^{-5}$ \\
%     \hline
%     \acro (Min) - PP 
%     \acro (Shift-All) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.448 & 98.480 $\pm$ 7.898 & 75.812 $\pm$ 24.337 & (1.337 $\pm$ 4.428) $\times 10^{-7}$ \\
%     \acro (QP) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.447 & 98.480 $\pm$ 7.898 & 75.812 $\pm$ 24.337 & (1.333 $\pm$ 4.423) $\times 10^{-7}$ \\
%     \hline
%     \acro (Min) - Optim 
%     \acro (Shift-All) - Optim &
%     \acro (QP) - Optim & 
%     \hline
%     \acro (Min) - Train
%     \acro (Shift-All) - Train & 1.161 $\pm$ 5.533 & 88.137 $\pm$ 12.256 & 98.636 $\pm$ 7.216 & 76.435 $\pm$ 24.276 & (2.418 $\pm$ 11.320) $\times 10^{-8}$ \\
%     \acro (QP) - Train & 1.289 $\pm$ 6.767 & 88.032 $\pm$ 12.619 & 98.621 $\pm$ 7.950 & 76.419 $\pm$ 24.389 & (6.174 $\pm$ 25.820) $\times 10^{-9}$ \\
%  \end{tabular}%
% }
% \caption{Shape reconstruction metrics for PartSDF on 100 mixers from the test set. Mean and standard deviations across shapes and parts.}
% \label{tab:partsdf_mixer100}
% \end{table}

==> tabs/supp_objectsdfplus_scenes_all.tex <==
% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|cccc}
%      & MCD ($\times 10^{-2}$) $\downarrow$ & NC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ \\
%     \hline
%     Vanilla ObjectSDF++         & $5.497 \pm 15.830$ & $0.786 \pm 0.104$ & $0.857 \pm 0.143$ & $1.438 \pm 3.757 (\times 10^{-3})$ \\
%     \hline
%     \acro{} (Min) - PP             & $3.280 \pm 11.823$ & $0.786 \pm 0.104$ & $0.868 \pm 0.138$ & $4.455 \pm 22.704 (\times 10^{-7})$ \\
%     \acro{} (MultiSDF)- PP & $3.813 \pm 13.120$ & $0.780 \pm 0.106$ & $0.864 \pm 0.142$ & $2.868 \pm 7.918 (\times 10^{-6})$ \\
%     \acro{} (QP) - PP              & $3.095 \pm 11.093$ & $0.786 \pm 0.104$ & $0.869 \pm 0.138$ & $1.046 \pm 5.279 (\times 10^{-7})$ \\
%     \acro{} (Shift-All) - PP           & $3.183 \pm 11.474$ & $0.787 \pm 0.107$ & $0.869 \pm 0.138$ & $1.124 \pm 4.423 (\times 10^{-7})$ \\
%     \hline
%     \acro{} (Shift-All Eikonal) - Train/PP   & $4.795 \pm 26.764$ & $0.768 \pm 0.110$ & $0.860 \pm 0.153$ & $2.436 \pm 10.266 (\times 10^{-7})$ \\
%     \acro{} (Shift-All Partial) - Train/PP    & $1.847 \pm 24.549$ & $0.768 \pm 0.102$ & $0.829 \pm 0.171$ & $2.877 \pm 25.094 (\times 10^{-7})$ \\
%   \end{tabular}%
% }
% \caption{ObjectSDF++~\cite{Wu23b} trained for object-compositional 3D scene reconstruction on 8 Replica~\cite{Straub19} scenes. Mean metrics across scenes and objects, weighted by the number of objects per scene.}
% \label{tab:supp_objectsdfplus_scenes_all}%
% \end{table}


\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{c|cccc}
     & MCD ($\times 10^{-2}$) $\downarrow$ & NC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ \\
    \hline
    Vanilla ObjectSDF++         & $5.497 \pm 15.830$ & $0.786 \pm 0.104$ & $0.857 \pm 0.143$ & $1.438 \pm 3.757 (\times 10^{-3})$ \\
    \hline
    \acro{} (Min) - PP             & $3.280 \pm 11.823$ & $0.786 \pm 0.104$ & $0.868 \pm 0.138$ & $4.455 \pm 22.704 (\times 10^{-7})$ \\
    \acro{} (QP) - PP              & $3.095 \pm 11.093$ & $0.786 \pm 0.104$ & $0.869 \pm 0.138$ & $1.046 \pm 5.279 (\times 10^{-7})$ \\
    \acro{} (Shift-All) - PP           & $3.183 \pm 11.474$ & $0.787 \pm 0.107$ & $0.869 \pm 0.138$ & $1.124 \pm 4.423 (\times 10^{-7})$ \\
  \end{tabular}%
}
\caption{ObjectSDF++~\cite{Wu23b} trained for object-compositional 3D scene reconstruction on 8 Replica~\cite{Straub19} scenes. Mean metrics across scenes and objects, weighted by the number of objects per scene.}
\label{tab:supp_objectsdfplus_scenes_all}%
\end{table}

==> tabs/supp_objectsdfplus_scenes_all_nobg.tex <==

\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{c|cccc}
     & MCD ($\times 10^{-2}$) $\downarrow$ & NC $\uparrow$ & F1 (0.01) $\uparrow$ & IV $\downarrow$ \\
    \hline
    Vanilla ObjectSDF++ & $9.716 \pm 5.602$ & $77.393 \pm 0.318$ & $66.801 \pm 0.114$ & $(1.447 \pm 0.128) \times 10^{-3}$ \\
    \hline
    \acro{} (QP) - PP & $2.919 \pm 0.866$ & $77.464 \pm 0.202$ & $68.190 \pm 0.198$ & $(1.908 \pm 0.606) \times 10^{-7}$ \\
    \acro{} (Shift-All) - PP & $2.085 \pm 0.236$ & $77.500 \pm 0.188$ & $68.242 \pm 0.182$ & $(1.315 \pm 0.246) \times 10^{-7}$ \\
    \hline
    \acro{} (Shift-All) - Train & $4.730 \pm 1.007$ & $75.861 \pm 0.237$ & $66.710 \pm 0.765$ & $(2.363 \pm 0.206) \times 10^{-7}$ \\
    \acro{} (Shift-All Skip-Conn.) - Train & $3.186 \pm 1.106$ & $77.847 \pm 0.515$ & $68.525 \pm 0.705$ & $(1.550 \pm 1.999) \times 10^{-6}$ \\
  \end{tabular}%
}
\caption{ObjectSDF++~\cite{Wu23b} trained for object-compositional 3D scene reconstruction on 8 Replica~\cite{Straub19} scenes. Mean and standard deviation across 3 runs. Background mesh has been excluded from the evaluation due to the presence of large surfaces outside of the scenes across all methods, which could skew the metrics and make them less informative.}
\label{tab:supp_objectsdfplus_scenes_all_nobg}%
\end{table}

==> tabs/supp_partsdf_chair.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{c|cccccc}
     & MCD $\downarrow$ & NC $\uparrow$ & F1 (0.001) $\uparrow$ & F1 (0.005) $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
    \hline
    Vanilla (MC) & 2.644 $\pm$ 6.492 & 96.237 $\pm$ 2.251 & 97.264 $\pm$ 3.441 & 99.307 $\pm$ 1.957 & 89.789 $\pm$ 8.545 & (1.230 $\pm$ 3.704) $\times 10^{-3}$ \\
    \hline
    Min - PP (MC) & 1.393 $\pm$ 2.496 & 96.062 $\pm$ 2.357 & 98.223 $\pm$ 2.066 & 99.721 $\pm$ 0.832 & 92.694 $\pm$ 5.656 & (1.479 $\pm$ 2.620) $\times 10^{-7}$ \\
    Shift - PP (MC) & 1.353 $\pm$ 2.411 & 96.181 $\pm$ 2.312 & 98.282 $\pm$ 2.007 & 99.729 $\pm$ 0.805 & 92.646 $\pm$ 5.705 & (1.917 $\pm$ 5.299) $\times 10^{-8}$ \\
    QP - PP (MC) & 1.358 $\pm$ 2.434 & 96.178 $\pm$ 2.315 & 98.275 $\pm$ 2.015 & 99.728 $\pm$ 0.810 & 92.640 $\pm$ 5.707 & (2.316 $\pm$ 10.350) $\times 10^{-8}$ \\
    \hline
    Min - Train (MC) & 1.510 $\pm$ 2.919 & 96.076 $\pm$ 2.312 & 98.151 $\pm$ 2.124 & 99.681 $\pm$ 0.946 & 92.607 $\pm$ 5.654 & (1.814 $\pm$ 3.617) $\times 10^{-7}$ \\
    Shift - Train (MC) & 1.580 $\pm$ 2.758 & 96.080 $\pm$ 2.279 & 98.060 $\pm$ 2.308 & 99.633 $\pm$ 1.056 & 92.341 $\pm$ 6.179 & (8.743 $\pm$ 17.980) $\times 10^{-8}$ \\
    QP - Train (MC) & 1.687 $\pm$ 4.706 & 96.108 $\pm$ 2.196 & 98.114 $\pm$ 2.229 & 99.653 $\pm$ 1.029 & 92.350 $\pm$ 6.119 & (9.055 $\pm$ 18.070) $\times 10^{-8}$ \\
  \end{tabular}%
}
\caption{PartSDF trained on all chairs in the training set (like in the original paper), tested on different 100 chairs. Mean metrics across shapes and parts (issue in the evaluation, disregard for now).}
\label{tab:supp_partsdf_chair_all}%
\end{table}

==> tabs/supp_partsdf_chair100_all.tex <==
% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|ccccccccc}
%      & MCD $\downarrow$ & Comp $\downarrow$ & Acc $\downarrow$ & NC $\uparrow$ & F1 (0.01) $\uparrow$ & F1 (0.05) $\uparrow$ & Proximal CD $\downarrow$ & IV $\downarrow$ & IoU $\uparrow$ \\
%     \hline
%     Vanilla (MC) & 3.567 $\times 10^{-4}$ & 3.288 $\times 10^{-4}$ & 2.799 $\times 10^{-5}$ & 9.511 $\times 10^{-1}$ & 9.973 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.208 $\times 10^{-4}$ & 1.788 $\times 10^{-3}$ & 8.572 $\times 10^{-1}$\\
%     Vanilla (MT) & 3.583 $\times 10^{-4}$ & 3.306 $\times 10^{-4}$ & 2.767 $\times 10^{-5}$ & 9.509 $\times 10^{-1}$ & 9.972 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.209 $\times 10^{-4}$ & 1.788 $\times 10^{-3}$ & 8.578 $\times 10^{-1}$\\
%     \hline
%     Min - PP (MC) & 2.249 $\times 10^{-4}$ & 1.938 $\times 10^{-4}$ & 3.110 $\times 10^{-5}$ & 9.474 $\times 10^{-1}$ & 9.987 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.372 $\times 10^{-4}$ & 1.454 $\times 10^{-7}$ & 8.921 $\times 10^{-1}$ \\
%     Min - PP (MT) & 2.308 $\times 10^{-4}$ & 2.005 $\times 10^{-4}$ & 3.034 $\times 10^{-5}$ & 9.459 $\times 10^{-1}$ & 9.987 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.271 $\times 10^{-4}$ & 5.150 $\times 10^{-12}$ & 8.925 $\times 10^{-1}$ \\
%     Shift - PP (MC) & 2.206 $\times 10^{-4}$ & 1.890 $\times 10^{-4}$ & 3.163 $\times 10^{-5}$ & 9.483 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.472 $\times 10^{-4}$ & 6.663 $\times 10^{-9}$ & 8.921 $\times 10^{-1}$ \\
%     Shift - PP (MT) & 2.525 $\times 10^{-4}$ & 2.214 $\times 10^{-4}$ & 3.117 $\times 10^{-5}$ & 9.481 $\times 10^{-1}$ & 9.987 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.423 $\times 10^{-4}$ & 1.888 $\times 10^{-10}$ & 8.929 $\times 10^{-1}$ \\
%     QP - PP (MC) & 2.305 $\times 10^{-4}$ & 1.989 $\times 10^{-4}$ & 3.154 $\times 10^{-5}$ & 9.479 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.326 $\times 10^{-4}$ & 6.139 $\times 10^{-9}$ & 8.919 $\times 10^{-1}$ \\
%     QP - PP (MT) & 2.323 $\times 10^{-4}$ & 2.012 $\times 10^{-4}$ & 3.112 $\times 10^{-5}$ & 9.476 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.276 $\times 10^{-4}$ & 1.570 $\times 10^{-10}$ & 8.926 $\times 10^{-1}$ \\
%     \hline
%     Min - Optim (MC) & 2.244 $\times 10^{-4}$ & 1.888 $\times 10^{-4}$ & 3.561 $\times 10^{-5}$ & 9.471 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.999 $\times 10^{-1}$ & 4.282 $\times 10^{-4}$ & 1.681 $\times 10^{-7}$ & 8.907 $\times 10^{-1}$ \\
%     Min - Optim (MT) & 2.321 $\times 10^{-4}$ & 1.972 $\times 10^{-4}$ & 3.485 $\times 10^{-5}$ & 9.455 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.999 $\times 10^{-1}$ & 4.232 $\times 10^{-4}$ & 5.492 $\times 10^{-8}$ & 8.911 $\times 10^{-1}$ \\
%     Shift - Optim (MC) & 2.838 $\times 10^{-4}$ & 2.460 $\times 10^{-4}$ & 3.781 $\times 10^{-5}$ & 9.490 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.242 $\times 10^{-4}$ & 3.550 $\times 10^{-9}$ & 8.969 $\times 10^{-1}$ \\
%     Shift - Optim (MT) & 2.841 $\times 10^{-4}$ & 2.465 $\times 10^{-4}$ & 3.766 $\times 10^{-5}$ & 9.488 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.195 $\times 10^{-4}$ & 1.808 $\times 10^{-10}$ & 8.978 $\times 10^{-1}$ \\
%     QP - Optim (MC) & 2.801 $\times 10^{-4}$ & 2.354 $\times 10^{-4}$ & 4.471 $\times 10^{-5}$ & 9.487 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.240 $\times 10^{-4}$ & 4.145 $\times 10^{-9}$ & 8.963 $\times 10^{-1}$ \\
%     QP - Optim (MT) & 2.801 $\times 10^{-4}$ & 2.355 $\times 10^{-4}$ & 4.454 $\times 10^{-5}$ & 9.484 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.213 $\times 10^{-4}$ & 1.471 $\times 10^{-10}$ & 8.971 $\times 10^{-1}$ \\
%     \hline
%     Min - Train (MC) & 2.347 $\times 10^{-4}$ & 1.974 $\times 10^{-4}$ & 3.737 $\times 10^{-5}$ & 9.473 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.940 $\times 10^{-4}$ & 1.398 $\times 10^{-7}$ & 8.904 $\times 10^{-1}$ \\
%     Min - Train (MT) & 2.385 $\times 10^{-4}$ & 1.963 $\times 10^{-4}$ & 4.221 $\times 10^{-5}$ & 9.462 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 5.215 $\times 10^{-4}$ & 2.163 $\times 10^{-14}$ & 8.908 $\times 10^{-1}$ \\
%     Shift - Train (MC) & 2.173 $\times 10^{-4}$ & 1.901 $\times 10^{-4}$ & 2.720 $\times 10^{-5}$ & 9.480 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.459 $\times 10^{-4}$ & 7.320 $\times 10^{-9}$ & 8.920 $\times 10^{-1}$ \\
%     Shift - Train (MT) & 2.184 $\times 10^{-4}$ & 1.916 $\times 10^{-4}$ & 2.685 $\times 10^{-5}$ & 9.473 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.421 $\times 10^{-4}$ & 2.080 $\times 10^{-10}$ & 8.913 $\times 10^{-1}$ \\
%     QP - Train (MC) & 2.700 $\times 10^{-4}$ & 2.373 $\times 10^{-4}$ & 3.272 $\times 10^{-5}$ & 9.499 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.885 $\times 10^{-4}$ & 8.117 $\times 10^{-9}$ & 8.942 $\times 10^{-1}$ \\
%     QP - Train (MT) & 3.011 $\times 10^{-4}$ & 2.437 $\times 10^{-4}$ & 5.738 $\times 10^{-5}$ & 9.491 $\times 10^{-1}$ & 9.983 $\times 10^{-1}$ & 9.995 $\times 10^{-1}$ & 5.444 $\times 10^{-4}$ & 1.375 $\times 10^{-10}$ & 8.945 $\times 10^{-1}$ \\
%   \end{tabular}%
% }
% \caption{PartSDF trained on 100 chairs, tested on different 100 chairs. Mean metrics across shapes and parts.}
% \label{tab:supp_partsdf_chair100_all}%
% \end{table}

% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|ccccccccc}
%      & MCD $\downarrow$ & Comp $\downarrow$ & Acc $\downarrow$ & NC $\uparrow$ & F1 (0.01) $\uparrow$ & F1 (0.05) $\uparrow$ & Proximal CD $\downarrow$ & IV $\downarrow$ & IoU $\uparrow$ \\
%     \hline
%     Vanilla (MC) & 3.567 $\times 10^{-4}$ & 3.288 $\times 10^{-4}$ & 2.799 $\times 10^{-5}$ & 9.511 $\times 10^{-1}$ & 9.973 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.208 $\times 10^{-4}$ & 1.788 $\times 10^{-3}$ & 8.572 $\times 10^{-1}$\\
%     % Vanilla (MT) & 3.583 $\times 10^{-4}$ & 3.306 $\times 10^{-4}$ & 2.767 $\times 10^{-5}$ & 9.509 $\times 10^{-1}$ & 9.972 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.209 $\times 10^{-4}$ & 1.788 $\times 10^{-3}$ & 8.578 $\times 10^{-1}$\\
%     \hline
%     Min - PP (MC) & 2.249 $\times 10^{-4}$ & 1.938 $\times 10^{-4}$ & 3.110 $\times 10^{-5}$ & 9.474 $\times 10^{-1}$ & 9.987 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.372 $\times 10^{-4}$ & 1.454 $\times 10^{-7}$ & 8.921 $\times 10^{-1}$ \\
%     % Min - PP (MT) & 2.308 $\times 10^{-4}$ & 2.005 $\times 10^{-4}$ & 3.034 $\times 10^{-5}$ & 9.459 $\times 10^{-1}$ & 9.987 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.271 $\times 10^{-4}$ & 5.150 $\times 10^{-12}$ & 8.925 $\times 10^{-1}$ \\
%     Shift - PP (MC) & 2.206 $\times 10^{-4}$ & 1.890 $\times 10^{-4}$ & 3.163 $\times 10^{-5}$ & 9.483 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.472 $\times 10^{-4}$ & 6.663 $\times 10^{-9}$ & 8.921 $\times 10^{-1}$ \\
%     % Shift - PP (MT) & 2.525 $\times 10^{-4}$ & 2.214 $\times 10^{-4}$ & 3.117 $\times 10^{-5}$ & 9.481 $\times 10^{-1}$ & 9.987 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.423 $\times 10^{-4}$ & 1.888 $\times 10^{-10}$ & 8.929 $\times 10^{-1}$ \\
%     QP - PP (MC) & 2.305 $\times 10^{-4}$ & 1.989 $\times 10^{-4}$ & 3.154 $\times 10^{-5}$ & 9.479 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.326 $\times 10^{-4}$ & 6.139 $\times 10^{-9}$ & 8.919 $\times 10^{-1}$ \\
%     % QP - PP (MT) & 2.323 $\times 10^{-4}$ & 2.012 $\times 10^{-4}$ & 3.112 $\times 10^{-5}$ & 9.476 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.276 $\times 10^{-4}$ & 1.570 $\times 10^{-10}$ & 8.926 $\times 10^{-1}$ \\
%     \hline
%     Min - Optim (MC) & 2.244 $\times 10^{-4}$ & 1.888 $\times 10^{-4}$ & 3.561 $\times 10^{-5}$ & 9.471 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.999 $\times 10^{-1}$ & 4.282 $\times 10^{-4}$ & 1.681 $\times 10^{-7}$ & 8.907 $\times 10^{-1}$ \\
%     % Min - Optim (MT) & 2.321 $\times 10^{-4}$ & 1.972 $\times 10^{-4}$ & 3.485 $\times 10^{-5}$ & 9.455 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.999 $\times 10^{-1}$ & 4.232 $\times 10^{-4}$ & 5.492 $\times 10^{-8}$ & 8.911 $\times 10^{-1}$ \\
%     Shift - Optim (MC) & 2.838 $\times 10^{-4}$ & 2.460 $\times 10^{-4}$ & 3.781 $\times 10^{-5}$ & 9.490 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.242 $\times 10^{-4}$ & 3.550 $\times 10^{-9}$ & 8.969 $\times 10^{-1}$ \\
%     % Shift - Optim (MT) & 2.841 $\times 10^{-4}$ & 2.465 $\times 10^{-4}$ & 3.766 $\times 10^{-5}$ & 9.488 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.195 $\times 10^{-4}$ & 1.808 $\times 10^{-10}$ & 8.978 $\times 10^{-1}$ \\
%     QP - Optim (MC) & 2.801 $\times 10^{-4}$ & 2.354 $\times 10^{-4}$ & 4.471 $\times 10^{-5}$ & 9.487 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.240 $\times 10^{-4}$ & 4.145 $\times 10^{-9}$ & 8.963 $\times 10^{-1}$ \\
%     % QP - Optim (MT) & 2.801 $\times 10^{-4}$ & 2.355 $\times 10^{-4}$ & 4.454 $\times 10^{-5}$ & 9.484 $\times 10^{-1}$ & 9.984 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.213 $\times 10^{-4}$ & 1.471 $\times 10^{-10}$ & 8.971 $\times 10^{-1}$ \\
%     \hline
%     Min - Train (MC) & 2.347 $\times 10^{-4}$ & 1.974 $\times 10^{-4}$ & 3.737 $\times 10^{-5}$ & 9.473 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.940 $\times 10^{-4}$ & 1.398 $\times 10^{-7}$ & 8.904 $\times 10^{-1}$ \\
%     % Min - Train (MT) & 2.385 $\times 10^{-4}$ & 1.963 $\times 10^{-4}$ & 4.221 $\times 10^{-5}$ & 9.462 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 5.215 $\times 10^{-4}$ & 2.163 $\times 10^{-14}$ & 8.908 $\times 10^{-1}$ \\
%     Shift - Train (MC) & 2.173 $\times 10^{-4}$ & 1.901 $\times 10^{-4}$ & 2.720 $\times 10^{-5}$ & 9.480 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.459 $\times 10^{-4}$ & 7.320 $\times 10^{-9}$ & 8.920 $\times 10^{-1}$ \\
%     % Shift - Train (MT) & 2.184 $\times 10^{-4}$ & 1.916 $\times 10^{-4}$ & 2.685 $\times 10^{-5}$ & 9.473 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 9.998 $\times 10^{-1}$ & 3.421 $\times 10^{-4}$ & 2.080 $\times 10^{-10}$ & 8.913 $\times 10^{-1}$ \\
%     QP - Train (MC) & 2.700 $\times 10^{-4}$ & 2.373 $\times 10^{-4}$ & 3.272 $\times 10^{-5}$ & 9.499 $\times 10^{-1}$ & 9.986 $\times 10^{-1}$ & 9.996 $\times 10^{-1}$ & 4.885 $\times 10^{-4}$ & 8.117 $\times 10^{-9}$ & 8.942 $\times 10^{-1}$ \\
%     % QP - Train (MT) & 3.011 $\times 10^{-4}$ & 2.437 $\times 10^{-4}$ & 5.738 $\times 10^{-5}$ & 9.491 $\times 10^{-1}$ & 9.983 $\times 10^{-1}$ & 9.995 $\times 10^{-1}$ & 5.444 $\times 10^{-4}$ & 1.375 $\times 10^{-10}$ & 8.945 $\times 10^{-1}$ \\
%   \end{tabular}%
% }
% \caption{PartSDF trained on 100 chairs, tested on different 100 chairs. Mean metrics across shapes and parts.}
% \label{tab:supp_partsdf_chair100_all}%
% \end{table}



\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{c|ccccc}
    & MCD $(\times 10^{-4})$ $\downarrow$ & NC $\uparrow$ & F1 (0.001) $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
    \hline
    Vanilla PartSDF & $3.567 \pm 13.130$ & $95.107 \pm 4.402$ & $96.790 \pm 3.851$ & $85.716 \pm 10.951$ & $(1.788 \pm 5.729) \times 10^{-3}$ \\
    \hline
    % \acro{} (Min) - PP & $2.249 \pm 12.658$ & $94.743 \pm 4.473$ & $97.933 \pm 3.226$ & $89.209 \pm 9.618$ & $(1.454 \pm 3.146) \times 10^{-7}$ \\
    \acro{} (Shift-All) - PP & $2.206 \pm 12.680$ & $94.834 \pm 4.472$ & $98.003 \pm 3.193$ & $89.207 \pm 9.606$ & $(6.663 \pm 30.730) \times 10^{-9}$ \\
    \acro{} (QP) - PP & $2.305 \pm 12.704$ & $94.791 \pm 4.483$ & $97.915 \pm 3.278$ & $89.186 \pm 9.604$ & $(6.139 \pm 34.630) \times 10^{-9}$ \\
    \hline
    % \acro{} (Min) - Optim & $2.244 \pm 10.445$ & $94.708 \pm 4.579$ & $97.870 \pm 3.284$ & $89.071 \pm 9.570$ & $(1.681 \pm 3.408) \times 10^{-7}$ \\
    \acro{} (Shift-All) - Optim & $2.838 \pm 21.485$ & $94.898 \pm 4.474$ & $98.110 \pm 3.338$ & $89.686 \pm 9.737$ & $(3.550 \pm 32.310) \times 10^{-9}$ \\
    \acro{} (QP) - Optim & $2.801 \pm 20.365$ & $94.871 \pm 4.388$ & $98.081 \pm 3.254$ & $89.628 \pm 9.801$ & $(4.145 \pm 27.200) \times 10^{-9}$ \\
    \hline
    % \acro{} (Min) - Train & $2.347 \pm 12.954$ & $94.727 \pm 4.474$ & $97.922 \pm 3.133$ & $89.043 \pm 9.406$ & $(1.398 \pm 3.071) \times 10^{-7}$ \\
    \acro{} (Shift-All) - Train & $2.173 \pm 11.984$ & $94.800 \pm 4.437$ & $98.063 \pm 3.169$ & $89.196 \pm 9.407$ & $(7.320 \pm 26.150) \times 10^{-9}$ \\
    \acro{} (QP) - Train & $2.700 \pm 18.035$ & $94.991 \pm 4.085$ & $98.089 \pm 3.032$ & $89.416 \pm 9.361$ & $(8.117 \pm 40.900) \times 10^{-9}$ \\
 \end{tabular}%
}
\caption{Shape reconstruction metrics for PartSDF on 100 chairs from the test set. Mean and standard deviations across shapes and parts.}
\label{tab:partsdf_chair100_old1run}
\end{table}

==> tabs/supp_partsdf_mixer100_all.tex <==
% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|ccccccccc}
%      & MCD $\downarrow$ & Comp $\downarrow$ & Acc $\downarrow$ & NC $\uparrow$ & F1 (0.01) $\uparrow$ & F1 (0.05) $\uparrow$ & Proximal CD $\downarrow$ & IV $\downarrow$ & IoU $\uparrow$ \\
%     \hline
%     Vanilla (MC) & 1.298 $\times 10^{-4}$ & 4.495 $\times 10^{-6}$ & 1.253 $\times 10^{-4}$ & 8.810 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 7.059 $\times 10^{-4}$ & 4.005 $\times 10^{-5}$ & 7.667 $\times 10^{-1}$ \\
%     \hline
%     Min - PP (MC) & 1.296 $\times 10^{-4}$ & 4.251 $\times 10^{-6}$ & 1.253 $\times 10^{-4}$ & 8.818 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 7.055 $\times 10^{-4}$ & 1.470 $\times 10^{-7}$ & 7.673 $\times 10^{-1}$ \\
%     Shift - PP (MC) & 1.300 $\times 10^{-4}$ & 4.417 $\times 10^{-6}$ & 1.256 $\times 10^{-4}$ & 8.805 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 7.082 $\times 10^{-4}$ & 1.337 $\times 10^{-7}$ & 7.581 $\times 10^{-1}$ \\
%     QP - PP (MC) & 1.300 $\times 10^{-4}$ & 4.417 $\times 10^{-6}$ & 1.256 $\times 10^{-4}$ & 8.805 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 7.082 $\times 10^{-4}$ & 1.333 $\times 10^{-7}$ & 7.581 $\times 10^{-1}$ \\
%     \hline
%     Min - Optim (MC)  & 1.298 $\times 10^{-4}$ & 4.272 $\times 10^{-6}$ & 1.255 $\times 10^{-4}$ & 8.818 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 7.101 $\times 10^{-4}$ & 1.211 $\times 10^{-7}$ & 7.673 $\times 10^{-1}$ \\
%     Shift - Optim (MC) & 1.296 $\times 10^{-4}$ & 4.419 $\times 10^{-6}$ & 1.252 $\times 10^{-4}$ & 8.814 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 8.573 $\times 10^{-4}$ & 3.974 $\times 10^{-9}$ & 7.648 $\times 10^{-1}$ \\
%     QP - Optim (MC) & 1.303 $\times 10^{-4}$ & 4.432 $\times 10^{-6}$ & 1.258 $\times 10^{-4}$ & 8.813 $\times 10^{-1}$ & 9.988 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 8.626 $\times 10^{-4}$ & 4.101 $\times 10^{-9}$ & 7.648 $\times 10^{-1}$ \\
%     \hline
%     Min - Train (MC) & 1.497 $\times 10^{-4}$ & 5.489 $\times 10^{-6}$ & 1.442 $\times 10^{-4}$ & 8.813 $\times 10^{-1}$ & 9.983 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 7.904 $\times 10^{-4}$ & 3.740 $\times 10^{-9}$ & 7.680 $\times 10^{-1}$ \\
%     Shift - Train (MC) & 1.161 $\times 10^{-4}$ & 4.630 $\times 10^{-6}$ & 1.115 $\times 10^{-4}$ & 8.814 $\times 10^{-1}$ & 9.990 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 6.997 $\times 10^{-4}$ & 2.418 $\times 10^{-8}$ & 7.643 $\times 10^{-1}$ \\
%     QP - Train (MC) & 1.289 $\times 10^{-4}$ & 3.845 $\times 10^{-6}$ & 1.251 $\times 10^{-4}$ & 8.803 $\times 10^{-1}$ & 9.983 $\times 10^{-1}$ & 1.000 $\times 10^{0}$ & 7.631 $\times 10^{-4}$ & 6.174 $\times 10^{-9}$ & 7.642 $\times 10^{-1}$ \\
%   \end{tabular}%
% }
% \caption{PartSDF trained on 100 mixers, tested on different 100 mixers. Mean metrics across shapes and parts.}
% \label{tab:supp_partsdf_mixer100_all}
% \end{table}

% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
%   \begin{tabular}{c|ccccc}
%     & MCD $(\times 10^{-4})$ $\downarrow$ & NC $\uparrow$ & F1 (0.001) $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
%     \hline
%     Vanilla PartSDF & 1.298 $\pm$ 6.284 & 88.102 $\pm$ 12.363 & 98.481 $\pm$ 7.898 & 76.667 $\pm$ 23.994 & (4.005 $\pm$ 7.699) $\times 10^{-5}$ \\
%     \hline
%     S2MDF (QP) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.447 & 98.480 $\pm$ 7.898 & 75.812 $\pm$ 24.337 & (1.333 $\pm$ 4.423) $\times 10^{-7}$ \\
%     S2MDF (Shift-All) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.448 & 98.480 $\pm$ 7.898 & 75.812 $\pm$ 24.337 & (1.337 $\pm$ 4.428) $\times 10^{-7}$ \\
%     \hline
%     S2MDF (QP) - Train & 1.289 $\pm$ 6.767 & 88.032 $\pm$ 12.619 & 98.621 $\pm$ 7.950 & 76.419 $\pm$ 24.389 & (6.174 $\pm$ 25.820) $\times 10^{-9}$ \\
%     S2MDF (Shift-All) - Train & 1.161 $\pm$ 5.533 & 88.137 $\pm$ 12.256 & 98.636 $\pm$ 7.216 & 76.435 $\pm$ 24.276 & (2.418 $\pm$ 11.320) $\times 10^{-8}$ \\
%   \end{tabular}%
% }
% \caption{}
% \label{tab:supp_partsdf_mixer100}
% \end{table}


\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{c|ccccc}
    & MCD $(\times 10^{-4})$ $\downarrow$ & NC $\uparrow$ & F1 (0.001) $\uparrow$ & IoU $\uparrow$ & IV $\downarrow$ \\
    \hline
    Vanilla PartSDF & 1.298 $\pm$ 6.284 & 88.102 $\pm$ 12.363 & 98.481 $\pm$ 7.898 & 76.667 $\pm$ 23.994 & (4.005 $\pm$ 7.699) $\times 10^{-5}$ \\
    \hline
    % \acro{} (Min) - PP & $1.296 \pm 6.284$ & $88.182 \pm 12.416$ & $98.481 \pm 7.898$ & $76.734 \pm 24.043$ & $(1.470 \pm 5.412) \times 10^{-7}$ \\
    \acro{} (Shift-All) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.448 & 98.480 $\pm$ 7.898 & 75.812 $\pm$ 24.337 & (1.337 $\pm$ 4.428) $\times 10^{-7}$ \\
    \acro{} (QP) - PP & 1.300 $\pm$ 6.284 & 88.051 $\pm$ 12.447 & 98.480 $\pm$ 7.898 & 75.812 $\pm$ 24.337 & (1.333 $\pm$ 4.423) $\times 10^{-7}$ \\
    \hline
    % \acro{} (Min) - Optim & $1.298 \pm 6.290$ & $88.178 \pm 12.441$ & $98.477 \pm 7.940$ & $76.729 \pm 24.055$ & $(1.211 \pm 4.632) \times 10^{-7}$ \\
    \acro{} (Shift-All) - Optim & $1.296 \pm 6.208$ & $88.137 \pm 12.392$ & $98.481 \pm 7.868$ & $76.483 \pm 24.039$ & $(3.974 \pm 28.770) \times 10^{-9}$ \\
    \acro{} (QP) - Optim & $1.303 \pm 6.240$ & $88.129 \pm 12.405$ & $98.476 \pm 7.890$ & $76.482 \pm 24.037$ & $(4.101 \pm 28.890) \times 10^{-9}$ \\
    \hline
    % \acro{} (Min) - Train & $1.497 \pm 7.075$ & $88.133 \pm 12.645$ & $98.251 \pm 8.714$ & $76.801 \pm 24.015$ & $(3.740 \pm 19.160) \times 10^{-9}$ \\
    \acro{} (Shift-All) - Train & 1.161 $\pm$ 5.533 & 88.137 $\pm$ 12.256 & 98.636 $\pm$ 7.216 & 76.435 $\pm$ 24.276 & (2.418 $\pm$ 11.320) $\times 10^{-8}$ \\
    \acro{} (QP) - Train & 1.289 $\pm$ 6.767 & 88.032 $\pm$ 12.619 & 98.621 $\pm$ 7.950 & 76.419 $\pm$ 24.389 & (6.174 $\pm$ 25.820) $\times 10^{-9}$ \\
 \end{tabular}%
}
\caption{Shape reconstruction metrics for PartSDF on 100 mixers from the test set. Mean and standard deviations across shapes and parts.}
\label{tab:partsdf_mixer100_old1run}
\end{table}

==> tex/B_neurips_template.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\section{Submission of papers to NeurIPS 2026}


Please read the instructions below carefully and follow them faithfully.


\subsection{Style}


Papers to be submitted to NeurIPS 2026 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long, including figures. \textbf{Papers that exceed the page limit will not be reviewed (or in any other way considered) for presentation at the conference.}
Additional pages \emph{containing acknowledgments, references, checklist, and optional technical appendices} do not count as content pages. 


The margins in 2026 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the NeurIPS website as indicated below. Please make sure you use the current files and not previous versions. Tweaking the style files may be grounds for desk rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on the website at
\begin{center}
  \url{https://neurips.cc}.
\end{center}
% The file \verb+neurips_2026.pdf+ contains these instructions and illustrates the various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2026 is \verb+neurips_2026.sty+, rewritten for \LaTeXe{}. \textbf{Previous style files for \LaTeX{} 2.09,  Microsoft Word, and RTF are no longer supported.}


The \LaTeX{} style file contains three optional arguments: 
\begin{itemize}
\item \verb+final+, which creates a camera-ready copy, 
\item \verb+preprint+, which creates a preprint for submission to, e.g., arXiv, \item \verb+nonatbib+, which will not load the \verb+natbib+ package for you in case of package clash.
\end{itemize}


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the NeurIPS style, please use the \verb+preprint+ option. This will create a nonanonymized version of your work with the text ``Preprint. Work in progress.'' in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do not} use the \verb+final+ option, which should \textbf{only} be used for papers accepted to NeurIPS.


At submission time, please omit the \verb+final+ and \verb+preprint+ options. This will anonymize your submission and add line numbers to aid review. Please do \emph{not} refer to these line numbers in your paper as they will be removed during generation of camera-ready copies.


The file \verb+neurips_2026.tex+ may be used as a ``shell'' for writing your paper. All you have to do is replace the author, title, abstract, and text of the paper with your own.


The formatting instructions contained in these style files are summarized in Sections \cref{gen_inst}, \cref{headings}, and \cref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \cref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2026+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2026}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption. Explain what the figure shows and add a key take-away message to the caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
 reproduction purposes. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for the first word and proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean, and legible.  The table number and
title always appear before the table.  See Table~\cref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for the first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules}. We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\cref{sample-table}.


\begin{table}
  \caption{Sample table caption. Explain what the table shows and add a key take-away message to the caption.}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\approx$100     \\
    Axon     & Output terminal & $\approx$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes. Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ ``patterned'' shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2026/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix

\section{Technical appendices and supplementary material}
Technical appendices with additional results, figures, graphs, and proofs may be submitted with the paper submission before the full submission deadline (see above). You can upload a ZIP file for videos or code, but do not upload a separate PDF file for the appendix. There is no page limit for the technical appendices. 

Note: Think of the appendix as ``optional reading'' for reviewers. The paper must be able to stand alone without the appendix; for example, adding critical experiments that support the main claims to an appendix is inappropriate. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

